Debiased inference for proximal dose-response function

We study nonparametric inference for a continuous-treatment causal dose-response curve and its first derivative under unmeasured confounding, using treatment- and outcome-inducing proxies. We establish a proximal doubly robust pseudo-outcome whose conditional mean given treatment equals the dose-response curve whenever either bridge function is correctly specified. Their (smoothed) efficient influence function representations lead to cross-fitted local-polynomial estimators with explicit smoothing-bias correction. We establish pointwise and finite-dimensional asymptotic normality and oracle uniform Gaussian approximations over compact interior treatment intervals, allowing mean-squared-error-optimal bandwidths without undersmoothing. The derivative inference reuses the estimated bridges and the same form of bandwidth-dependent nuisance-rate conditions, evaluated at the bandwidth rate appropriate for derivative estimation, without requiring derivative-specific bridge estimation. Employing cross-fitting accommodates flexible bridge estimators under product convergence rate conditions without entropy restrictions. We further develop tests against fixed-dimensional parametric dose-response null hypotheses, including constancy, linearity, and quadratic specifications, and derive their limiting distributions under the null and local alternatives, together with practical bootstrap procedures. We also develop practical bandwidth selectors, pointwise confidence intervals, and simultaneous confidence bands for each causal estimand. Extensive simulations and a data analysis, presented in the appendix, demonstrate the finite-sample performance of the proposed methods under latent confounding and multiple proxies.

==> preamble-shared.tex <==
\usepackage[margin=1in]{geometry}
\usepackage[dvipsnames]{xcolor}
\usepackage{setspace,authblk,xparse}
\RequirePackage[authoryear]{natbib}
\usepackage{amssymb, amsmath, amsthm}
\usepackage{multirow}
\usepackage{booktabs,longtable,pdflscape}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{url}
\usepackage{enumitem}
\usepackage{pdfpages}
\usepackage{prodint}
\usepackage{mathrsfs}
\usepackage{fix-cm}
\usepackage{microtype}
\setlength{\emergencystretch}{5em}
% The official bibliography style emits this chapter-series field.
\providecommand{\bseriesno}[1]{#1}


% \usepackage{hyperref}

\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage{hypernat}

% \RequirePackage{makeidx}
\usepackage{imakeidx}
\makeindex

%% table packages
\usepackage{booktabs}
% \usepackage{slashbox}

% \usepackage[demo]{graphicx}
% % 


\makeatletter
\newcommand{\myitem}[1]{%
\item[#1]\protected@edef\@currentlabel{#1}%
}
\makeatother



\newcommand{\argmax}{\operatorname*{arg \ max}}
\newcommand{\argmin}{\operatorname*{arg \ min}}
\newcommand{\iid}{\stackrel{\text{iid}}{\sim}}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\DeclareMathOperator{\vol}{Vol}
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\diam}{diam}
\global\long\def\inv#1{\frac{1}{#1}}
\DeclareMathOperator*{\Bias}{Bias}
\DeclareMathOperator*{\MSE}{MSE}
\DeclareMathOperator*{\Cov}{Cov}
\DeclareMathOperator*{\Cor}{Cor}
\DeclareMathOperator*{\sd}{sd}
% \DeclareMathOperator*{\min}{min}
% \DeclareMathOperator*{\max}{max}
%% \mathrm is owrose than declaremathoperator
%\newcommand{\dom}{\mathrm{dom}}
%\newcommand{\sub}{\mathrm{sub}}

\usepackage{xcolor}

%%%commands for remark and modification %%%
\newcommand{\remHDY}[1]{{\noindent (\color{WildStrawberry}#1 --Daeyoung)} \index{HDY}}
\newcommand{\modHDY}[1]{{\noindent  \color{OliveGreen}#1} \index{HDY}}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\sub}{sub}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  Macros below here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\providecommand{\simfigdir}{figures/simulation}
\providecommand{\simtabledir}{tables/simulation}

\newcommand{\lp}{\left(} %% )
  \newcommand{\rp}{\right)}
\newcommand{\lb}{\left\{} %% )
  \newcommand{\rb}{\right\}}
\newcommand{\ls}{\left[} %% )
  \newcommand{\rs}{\right]}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}

\newcommand{\vp}{\varphi}


\newcommand{\ve}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\ve{#1}}

%% \newcommand{\cC}{\mathcal{C}} %% see below
\newcommand{\EE}{{\mathbb E}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\PPn}{{\mathbb P}_n}
\newcommand{\FFn}{{\mathbb F}_n}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\LL}{{\mathbb L}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\GGn}{{\mathbb G}_n}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\YY}{{\mathbb Y}}
\newcommand{\WW}{{\mathbb W}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{{\mathbb Z}}
\newcommand{\trainingsigma}{\mathscr{T}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}\mathrm{ar}}
\newcommand{\ind}{\mathbb{I}}
\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\given}{\,\middle|\,}
\newcommand{\m}{\mathrm{m}} % mediator value symbol
\newcommand{\x}{\mathrm{x}} % covariate value symbol
\newcommand{\ttt}{t}        % target t
\newcommand{\thh}{t+h} 

\newcommand{\I}{\mathcal{I}}
\newcommand{\K}{\mathcal{K}}

\newcommand{\ib}{\boldsymbol{i}}
\newcommand{\jb}{\boldsymbol{j}}
\newcommand{\Gb}{\boldsymbol{\Gamma}}



\newcommand{\eps}{\varepsilon}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\pp}{\ensuremath{\mathfrak{P}}}
% IMS uses \qq for template placeholders; preserve the manuscript's math macro.
\let\qq\undefined
\newcommand{\qq}{\ensuremath{\mathfrak{Q}}}
\newcommand{\mm}{\ensuremath{\mathfrak{M}}}
\newcommand{\ff}{\ensuremath{\mathcal {F}}}
\newcommand{\mbX}{\ensuremath{\mathbf {X}}}
\newcommand{\mbx}{\ensuremath{\mathbf {x}}}
\newcommand{\mbbeta}{\ensuremath{\pmb {\beta}}}
% \newcommand{\ff}{\ensuremath{\mathfrak{F}}}
\newcommand{\fft}{\ensuremath{\tilde{\mathfrak{F}}}}
\newcommand{\ffn}{\ensuremath{{\mathfrak{F}}^{\otimes n}}}
\newcommand{\ffb}{\ensuremath{\ff_{\text{BDD}}}}
\newcommand{\ffs}{\ensuremath{\ff_{\text{SMU}}}}


\newcommand{\one}{\mathbbm{1}}
\newcommand{\mc}[1]{\mathcal {#1}}
\newcommand{\bb}[1]{\mathbb {#1}}
\newcommand{\kl}[2]{\rho_{\mathrm{KL}}\left({#1} \, \Vert \, {#2} \right)}

% \newcommand{\argmin}{\mathrm{argmin}}
%%\newcommand{\inf}{\mathrm{inf}}
%%\newcommand{\sup}{\mathrm{sup}}
\newcommand{\limsupp}{{\overline{\mathrm{lim}}}}
%% \newcommand{\width}{{\mathrm{width}}}
\newcommand{\SPAN}{{\mathrm{span}}}

\newcommand{\linaff}{\operatorname{Lin}}
%% \newcommand{\lin}{{\mathrm{lin}}}
\newcommand{\Lin}{\operatorname{Lin}}

\theoremstyle{plain}
\newtheorem{alg}{Algorithm}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\theoremstyle{definition}
\newtheorem{defin}{Definition}
\newtheorem{assumption}{Assumption}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\theoremstyle{definition}
\newtheorem{remark}{Remark}

\renewcommand*{\theassumption}{\Alph{assumption}}

\newtheorem{assumptionalt}{Assumption}[assumption]

% New environment
\newenvironment{assumptionp}[1]{
  \renewcommand\theassumptionalt{#1}
  \assumptionalt
  \phantomsection
}{\endassumptionalt}


\bibliographystyle{asa}


% Shared JASA manuscript metadata and anonymous rendering.
\providecommand{\blind}{0}
\newcommand{\papertitle}{Debiased inference for proximal dose-response function}
\newcommand{\paperkeywords}{Debiased machine learning; Dose-response function; Efficient influence function; Proximal causal inference; Simultaneous confidence bands.}
\newcommand{\spacingset}[1]{\renewcommand{\baselinestretch}{#1}\small\normalsize}
\renewcommand\Authands{ and }
\date{}
\ifnum\blind=0
  \renewcommand{\remHDY}[1]{{\noindent (\color{WildStrawberry}#1)}}
\fi
% Keep the acknowledgement source intact; omit its body in anonymous PDFs.
\NewDocumentEnvironment{acks}{+b}{%
  \ifnum\blind=1
    \section*{Acknowledgments}#1\par
  \fi
}{}
\hypersetup{pdftitle={\papertitle},pdfauthor={},pdfsubject={},pdfkeywords={}}
\ifnum\blind=1
  \hypersetup{pdfauthor={Daeyoung Ham, Sihan Wu, Yifan Cui}}
\fi
% Allow single plot pages before their deferred queue blocks later figures.
\renewcommand{\floatpagefraction}{0.3}
\allowdisplaybreaks


==> tables/simulation/band-performance-rows.tex <==
% n & scenario & PDR-PI1 & PDR-PI2 & PDR-CV1 & PDR-CV2; coverage [mean width]
2500 & CC & 0.9484 [0.355] & 0.9558 [0.379] & 0.9488 [0.305] & 0.9450 [0.271] \\
2500 & CM & 0.9464 [0.351] & 0.9562 [0.373] & 0.9488 [0.300] & 0.9454 [0.268] \\
2500 & MC & 0.9386 [0.754] & 0.9414 [0.938] & 0.9360 [0.684] & 0.9354 [0.563] \\
2500 & MM & 0.1978 [0.703] & 0.3780 [0.872] & 0.1460 [0.634] & 0.0598 [0.521] \\
5000 & CC & 0.9424 [0.264] & 0.9498 [0.283] & 0.9444 [0.225] & 0.9450 [0.199] \\
5000 & CM & 0.9420 [0.261] & 0.9486 [0.278] & 0.9426 [0.222] & 0.9444 [0.196] \\
5000 & MC & 0.9428 [0.569] & 0.9486 [0.716] & 0.9436 [0.515] & 0.9410 [0.424] \\
5000 & MM & 0.0228 [0.534] & 0.1062 [0.669] & 0.0142 [0.481] & 0.0034 [0.396] \\
7500 & CC & 0.9450 [0.223] & 0.9484 [0.239] & 0.9446 [0.189] & 0.9392 [0.166] \\
7500 & CM & 0.9440 [0.220] & 0.9494 [0.235] & 0.9434 [0.186] & 0.9382 [0.164] \\
7500 & MC & 0.9420 [0.485] & 0.9464 [0.613] & 0.9440 [0.438] & 0.9450 [0.359] \\
7500 & MM & 0.0030 [0.456] & 0.0210 [0.573] & 0.0010 [0.410] & 0.0000 [0.334] \\
10000 & CC & 0.9488 [0.197] & 0.9526 [0.212] & 0.9470 [0.167] & 0.9432 [0.146] \\
10000 & CM & 0.9494 [0.194] & 0.9518 [0.209] & 0.9466 [0.164] & 0.9436 [0.144] \\
10000 & MC & 0.9402 [0.433] & 0.9462 [0.548] & 0.9420 [0.391] & 0.9466 [0.320] \\
10000 & MM & 0.0002 [0.407] & 0.0048 [0.513] & 0.0000 [0.366] & 0.0000 [0.300] \\
\bottomrule


==> tables/simulation/ci-nine-point-rows.tex <==
% n & scenario & method & nine cells, each coverage [mean width]
2500 & CC & PDR--PI1 & 0.950 [0.2678] & 0.947 [0.2500] & 0.952 [0.2370] & 0.954 [0.2305] & 0.946 [0.2288] & 0.948 [0.2306] & 0.948 [0.2370] & 0.946 [0.2501] & 0.950 [0.2683] \\
2500 & CC & PDR--PI2 & 0.953 [0.2818] & 0.954 [0.2620] & 0.952 [0.2474] & 0.954 [0.2400] & 0.948 [0.2380] & 0.952 [0.2401] & 0.950 [0.2474] & 0.949 [0.2620] & 0.952 [0.2824] \\
2500 & CC & PDR--CV1 & 0.955 [0.2382] & 0.951 [0.2249] & 0.956 [0.2152] & 0.954 [0.2103] & 0.951 [0.2091] & 0.947 [0.2104] & 0.949 [0.2152] & 0.943 [0.2249] & 0.947 [0.2385] \\
2500 & CC & PDR--CV2 & 0.953 [0.2190] & 0.949 [0.2089] & 0.951 [0.2017] & 0.952 [0.1979] & 0.947 [0.1970] & 0.946 [0.1980] & 0.944 [0.2016] & 0.943 [0.2089] & 0.946 [0.2192] \\
2500 & CC & ProxLL--US & 0.951 [0.3126] & 0.948 [0.2883] & 0.953 [0.2704] & 0.953 [0.2617] & 0.948 [0.2593] & 0.951 [0.2617] & 0.950 [0.2706] & 0.948 [0.2887] & 0.947 [0.3132] \\
2500 & MC & PDR--PI1 & 0.952 [0.6113] & 0.948 [0.5373] & 0.947 [0.4842] & 0.946 [0.4553] & 0.943 [0.4474] & 0.949 [0.4548] & 0.948 [0.4834] & 0.951 [0.5378] & 0.955 [0.6118] \\
2500 & MC & PDR--PI2 & 0.956 [0.7364] & 0.952 [0.6466] & 0.945 [0.5813] & 0.943 [0.5463] & 0.948 [0.5361] & 0.950 [0.5456] & 0.947 [0.5810] & 0.953 [0.6462] & 0.955 [0.7364] \\
2500 & MC & PDR--CV1 & 0.952 [0.5635] & 0.952 [0.4963] & 0.945 [0.4473] & 0.941 [0.4208] & 0.942 [0.4135] & 0.947 [0.4203] & 0.950 [0.4467] & 0.950 [0.4962] & 0.956 [0.5640] \\
2500 & MC & PDR--CV2 & 0.957 [0.4769] & 0.953 [0.4220] & 0.939 [0.3818] & 0.937 [0.3597] & 0.939 [0.3538] & 0.942 [0.3593] & 0.951 [0.3811] & 0.951 [0.4220] & 0.958 [0.4776] \\
2500 & MC & ProxLL--US & 0.956 [0.7629] & 0.949 [0.6688] & 0.948 [0.6006] & 0.950 [0.5636] & 0.947 [0.5537] & 0.951 [0.5635] & 0.946 [0.5999] & 0.954 [0.6703] & 0.953 [0.7632] \\
2500 & CM & PDR--PI1 & 0.951 [0.2661] & 0.947 [0.2492] & 0.951 [0.2367] & 0.953 [0.2300] & 0.944 [0.2278] & 0.947 [0.2287] & 0.948 [0.2333] & 0.945 [0.2434] & 0.950 [0.2574] \\
2500 & CM & PDR--PI2 & 0.953 [0.2789] & 0.953 [0.2604] & 0.953 [0.2463] & 0.953 [0.2388] & 0.948 [0.2363] & 0.951 [0.2372] & 0.950 [0.2425] & 0.946 [0.2537] & 0.953 [0.2693] \\
2500 & CM & PDR--CV1 & 0.953 [0.2361] & 0.951 [0.2236] & 0.957 [0.2144] & 0.954 [0.2095] & 0.951 [0.2079] & 0.945 [0.2086] & 0.948 [0.2120] & 0.943 [0.2194] & 0.947 [0.2298] \\
2500 & CM & PDR--CV2 & 0.951 [0.2174] & 0.950 [0.2079] & 0.950 [0.2011] & 0.953 [0.1973] & 0.946 [0.1962] & 0.945 [0.1966] & 0.943 [0.1993] & 0.945 [0.2049] & 0.944 [0.2127] \\
2500 & CM & ProxLL--US & 0.951 [0.3106] & 0.947 [0.2878] & 0.950 [0.2704] & 0.953 [0.2612] & 0.946 [0.2581] & 0.949 [0.2593] & 0.951 [0.2657] & 0.947 [0.2796] & 0.948 [0.2985] \\
2500 & MM & PDR--PI1 & 0.412 [0.5611] & 0.548 [0.5054] & 0.769 [0.4625] & 0.918 [0.4374] & 0.931 [0.4286] & 0.808 [0.4312] & 0.559 [0.4478] & 0.340 [0.4818] & 0.231 [0.5280] \\
2500 & MM & PDR--PI2 & 0.584 [0.6740] & 0.689 [0.6062] & 0.826 [0.5536] & 0.930 [0.5236] & 0.937 [0.5124] & 0.867 [0.5159] & 0.683 [0.5365] & 0.506 [0.5773] & 0.392 [0.6339] \\
2500 & MM & PDR--CV1 & 0.356 [0.5144] & 0.510 [0.4635] & 0.739 [0.4245] & 0.910 [0.4018] & 0.926 [0.3937] & 0.789 [0.3960] & 0.516 [0.4113] & 0.288 [0.4419] & 0.178 [0.4841] \\
2500 & MM & PDR--CV2 & 0.216 [0.4357] & 0.373 [0.3939] & 0.665 [0.3621] & 0.895 [0.3433] & 0.916 [0.3367] & 0.725 [0.3384] & 0.396 [0.3510] & 0.171 [0.3760] & 0.088 [0.4105] \\
2500 & MM & ProxLL--US & 0.575 [0.6980] & 0.698 [0.6277] & 0.829 [0.5722] & 0.935 [0.5402] & 0.935 [0.5293] & 0.863 [0.5328] & 0.676 [0.5544] & 0.494 [0.5973] & 0.387 [0.6566] \\
5000 & CC & PDR--PI1 & 0.950 [0.1966] & 0.947 [0.1828] & 0.953 [0.1731] & 0.948 [0.1680] & 0.955 [0.1666] & 0.954 [0.1680] & 0.951 [0.1731] & 0.951 [0.1829] & 0.955 [0.1966] \\
5000 & CC & PDR--PI2 & 0.953 [0.2081] & 0.948 [0.1927] & 0.954 [0.1817] & 0.953 [0.1760] & 0.955 [0.1744] & 0.954 [0.1760] & 0.948 [0.1818] & 0.950 [0.1928] & 0.957 [0.2081] \\
5000 & CC & PDR--CV1 & 0.949 [0.1736] & 0.950 [0.1633] & 0.951 [0.1560] & 0.949 [0.1523] & 0.955 [0.1513] & 0.956 [0.1523] & 0.947 [0.1561] & 0.955 [0.1633] & 0.950 [0.1736] \\
5000 & CC & PDR--CV2 & 0.951 [0.1586] & 0.951 [0.1507] & 0.951 [0.1452] & 0.949 [0.1424] & 0.958 [0.1416] & 0.954 [0.1424] & 0.950 [0.1452] & 0.953 [0.1508] & 0.950 [0.1586] \\
5000 & CC & ProxLL--US & 0.949 [0.2377] & 0.953 [0.2181] & 0.954 [0.2042] & 0.953 [0.1970] & 0.958 [0.1949] & 0.953 [0.1969] & 0.955 [0.2043] & 0.952 [0.2183] & 0.954 [0.2374] \\
5000 & MC & PDR--PI1 & 0.947 [0.4544] & 0.950 [0.4004] & 0.946 [0.3614] & 0.950 [0.3402] & 0.951 [0.3345] & 0.944 [0.3401] & 0.953 [0.3609] & 0.946 [0.4006] & 0.954 [0.4544] \\
5000 & MC & PDR--PI2 & 0.950 [0.5533] & 0.949 [0.4868] & 0.951 [0.4388] & 0.949 [0.4129] & 0.949 [0.4060] & 0.948 [0.4129] & 0.953 [0.4384] & 0.946 [0.4873] & 0.950 [0.5530] \\
5000 & MC & PDR--CV1 & 0.953 [0.4185] & 0.947 [0.3690] & 0.947 [0.3332] & 0.944 [0.3139] & 0.951 [0.3086] & 0.946 [0.3138] & 0.954 [0.3328] & 0.945 [0.3690] & 0.954 [0.4186] \\
5000 & MC & PDR--CV2 & 0.953 [0.3544] & 0.949 [0.3136] & 0.950 [0.2838] & 0.948 [0.2679] & 0.945 [0.2635] & 0.949 [0.2678] & 0.951 [0.2837] & 0.949 [0.3135] & 0.952 [0.3546] \\
5000 & MC & ProxLL--US & 0.947 [0.5875] & 0.947 [0.5164] & 0.953 [0.4652] & 0.954 [0.4370] & 0.947 [0.4300] & 0.950 [0.4371] & 0.954 [0.4642] & 0.950 [0.5162] & 0.954 [0.5868] \\
5000 & CM & PDR--PI1 & 0.947 [0.1959] & 0.946 [0.1826] & 0.952 [0.1730] & 0.947 [0.1677] & 0.953 [0.1659] & 0.954 [0.1665] & 0.951 [0.1703] & 0.953 [0.1779] & 0.952 [0.1885] \\
5000 & CM & PDR--PI2 & 0.951 [0.2064] & 0.948 [0.1918] & 0.955 [0.1810] & 0.951 [0.1751] & 0.955 [0.1730] & 0.954 [0.1737] & 0.948 [0.1779] & 0.952 [0.1864] & 0.954 [0.1982] \\
5000 & CM & PDR--CV1 & 0.949 [0.1725] & 0.950 [0.1627] & 0.952 [0.1556] & 0.949 [0.1517] & 0.956 [0.1504] & 0.955 [0.1509] & 0.946 [0.1537] & 0.952 [0.1593] & 0.949 [0.1672] \\
5000 & CM & PDR--CV2 & 0.948 [0.1576] & 0.949 [0.1502] & 0.951 [0.1448] & 0.948 [0.1419] & 0.957 [0.1410] & 0.954 [0.1413] & 0.951 [0.1434] & 0.951 [0.1477] & 0.950 [0.1537] \\
5000 & CM & ProxLL--US & 0.947 [0.2369] & 0.950 [0.2181] & 0.957 [0.2045] & 0.952 [0.1967] & 0.958 [0.1940] & 0.954 [0.1949] & 0.955 [0.2004] & 0.951 [0.2113] & 0.952 [0.2262] \\
5000 & MM & PDR--PI1 & 0.200 [0.4220] & 0.347 [0.3794] & 0.649 [0.3471] & 0.912 [0.3285] & 0.929 [0.3218] & 0.719 [0.3237] & 0.347 [0.3362] & 0.148 [0.3618] & 0.070 [0.3968] \\
5000 & MM & PDR--PI2 & 0.358 [0.5113] & 0.515 [0.4592] & 0.758 [0.4196] & 0.925 [0.3969] & 0.937 [0.3887] & 0.803 [0.3911] & 0.512 [0.4063] & 0.278 [0.4378] & 0.173 [0.4802] \\
5000 & MM & PDR--CV1 & 0.141 [0.3864] & 0.288 [0.3476] & 0.607 [0.3181] & 0.900 [0.3012] & 0.923 [0.2951] & 0.691 [0.2969] & 0.284 [0.3082] & 0.100 [0.3315] & 0.042 [0.3633] \\
5000 & MM & PDR--CV2 & 0.064 [0.3275] & 0.165 [0.2955] & 0.494 [0.2711] & 0.878 [0.2571] & 0.913 [0.2521] & 0.599 [0.2534] & 0.176 [0.2628] & 0.048 [0.2820] & 0.016 [0.3082] \\
5000 & MM & ProxLL--US & 0.390 [0.5453] & 0.539 [0.4890] & 0.771 [0.4467] & 0.925 [0.4220] & 0.938 [0.4133] & 0.807 [0.4159] & 0.532 [0.4323] & 0.299 [0.4657] & 0.207 [0.5121] \\
7500 & CC & PDR--PI1 & 0.949 [0.1648] & 0.943 [0.1530] & 0.948 [0.1447] & 0.946 [0.1403] & 0.947 [0.1392] & 0.947 [0.1404] & 0.948 [0.1447] & 0.947 [0.1531] & 0.948 [0.1649] \\
7500 & CC & PDR--PI2 & 0.952 [0.1746] & 0.944 [0.1614] & 0.950 [0.1521] & 0.946 [0.1471] & 0.952 [0.1458] & 0.952 [0.1472] & 0.952 [0.1520] & 0.948 [0.1614] & 0.950 [0.1746] \\
7500 & CC & PDR--CV1 & 0.947 [0.1447] & 0.944 [0.1358] & 0.947 [0.1296] & 0.945 [0.1263] & 0.949 [0.1255] & 0.947 [0.1264] & 0.953 [0.1296] & 0.946 [0.1358] & 0.946 [0.1446] \\
7500 & CC & PDR--CV2 & 0.946 [0.1315] & 0.943 [0.1247] & 0.947 [0.1200] & 0.944 [0.1176] & 0.947 [0.1170] & 0.946 [0.1176] & 0.952 [0.1201] & 0.948 [0.1248] & 0.945 [0.1315] \\
7500 & CC & ProxLL--US & 0.952 [0.2035] & 0.948 [0.1865] & 0.953 [0.1745] & 0.957 [0.1678] & 0.952 [0.1663] & 0.957 [0.1681] & 0.954 [0.1744] & 0.946 [0.1867] & 0.953 [0.2037] \\
7500 & MC & PDR--PI1 & 0.956 [0.3846] & 0.948 [0.3391] & 0.949 [0.3056] & 0.949 [0.2879] & 0.949 [0.2832] & 0.948 [0.2880] & 0.948 [0.3055] & 0.953 [0.3391] & 0.954 [0.3844] \\
7500 & MC & PDR--PI2 & 0.956 [0.4696] & 0.949 [0.4139] & 0.952 [0.3726] & 0.954 [0.3505] & 0.951 [0.3448] & 0.948 [0.3507] & 0.947 [0.3726] & 0.949 [0.4138] & 0.951 [0.4694] \\
7500 & MC & PDR--CV1 & 0.958 [0.3531] & 0.951 [0.3116] & 0.944 [0.2810] & 0.949 [0.2648] & 0.944 [0.2605] & 0.946 [0.2648] & 0.947 [0.2809] & 0.952 [0.3115] & 0.956 [0.3531] \\
7500 & MC & PDR--CV2 & 0.963 [0.2983] & 0.954 [0.2639] & 0.945 [0.2386] & 0.945 [0.2253] & 0.944 [0.2216] & 0.943 [0.2252] & 0.949 [0.2387] & 0.953 [0.2638] & 0.963 [0.2982] \\
7500 & MC & ProxLL--US & 0.956 [0.5066] & 0.953 [0.4460] & 0.953 [0.4009] & 0.954 [0.3774] & 0.947 [0.3711] & 0.953 [0.3777] & 0.952 [0.4012] & 0.954 [0.4461] & 0.953 [0.5065] \\
7500 & CM & PDR--PI1 & 0.945 [0.1641] & 0.941 [0.1528] & 0.948 [0.1445] & 0.944 [0.1399] & 0.948 [0.1384] & 0.947 [0.1389] & 0.949 [0.1421] & 0.946 [0.1486] & 0.946 [0.1578] \\
7500 & CM & PDR--PI2 & 0.947 [0.1734] & 0.944 [0.1607] & 0.953 [0.1515] & 0.946 [0.1463] & 0.951 [0.1446] & 0.952 [0.1452] & 0.953 [0.1487] & 0.946 [0.1560] & 0.949 [0.1662] \\
7500 & CM & PDR--CV1 & 0.942 [0.1437] & 0.942 [0.1352] & 0.947 [0.1292] & 0.945 [0.1258] & 0.950 [0.1247] & 0.947 [0.1251] & 0.951 [0.1275] & 0.948 [0.1323] & 0.946 [0.1391] \\
7500 & CM & PDR--CV2 & 0.942 [0.1308] & 0.943 [0.1244] & 0.948 [0.1198] & 0.941 [0.1173] & 0.946 [0.1165] & 0.945 [0.1168] & 0.950 [0.1186] & 0.946 [0.1222] & 0.946 [0.1274] \\
7500 & CM & ProxLL--US & 0.949 [0.2029] & 0.950 [0.1864] & 0.955 [0.1744] & 0.957 [0.1675] & 0.950 [0.1653] & 0.955 [0.1661] & 0.952 [0.1707] & 0.949 [0.1803] & 0.949 [0.1935] \\
7500 & MM & PDR--PI1 & 0.094 [0.3579] & 0.218 [0.3215] & 0.545 [0.2939] & 0.893 [0.2780] & 0.923 [0.2724] & 0.647 [0.2740] & 0.225 [0.2847] & 0.062 [0.3065] & 0.027 [0.3359] \\
7500 & MM & PDR--PI2 & 0.219 [0.4354] & 0.386 [0.3909] & 0.670 [0.3570] & 0.914 [0.3373] & 0.933 [0.3305] & 0.753 [0.3325] & 0.403 [0.3458] & 0.151 [0.3724] & 0.077 [0.4087] \\
7500 & MM & PDR--CV1 & 0.056 [0.3271] & 0.155 [0.2942] & 0.485 [0.2690] & 0.879 [0.2546] & 0.914 [0.2495] & 0.601 [0.2508] & 0.171 [0.2606] & 0.033 [0.2804] & 0.012 [0.3072] \\
7500 & MM & PDR--CV2 & 0.020 [0.2756] & 0.074 [0.2485] & 0.342 [0.2277] & 0.848 [0.2159] & 0.900 [0.2116] & 0.482 [0.2127] & 0.082 [0.2208] & 0.012 [0.2371] & 0.005 [0.2591] \\
7500 & MM & ProxLL--US & 0.270 [0.4715] & 0.427 [0.4225] & 0.700 [0.3856] & 0.922 [0.3642] & 0.933 [0.3568] & 0.770 [0.3590] & 0.440 [0.3734] & 0.205 [0.4026] & 0.117 [0.4420] \\
10000 & CC & PDR--PI1 & 0.948 [0.1451] & 0.946 [0.1346] & 0.950 [0.1270] & 0.948 [0.1231] & 0.946 [0.1220] & 0.951 [0.1231] & 0.947 [0.1270] & 0.946 [0.1345] & 0.953 [0.1450] \\
10000 & CC & PDR--PI2 & 0.949 [0.1544] & 0.948 [0.1426] & 0.952 [0.1340] & 0.949 [0.1296] & 0.949 [0.1284] & 0.955 [0.1296] & 0.951 [0.1340] & 0.946 [0.1425] & 0.957 [0.1543] \\
10000 & CC & PDR--CV1 & 0.945 [0.1272] & 0.941 [0.1193] & 0.951 [0.1136] & 0.950 [0.1107] & 0.947 [0.1099] & 0.953 [0.1107] & 0.949 [0.1136] & 0.949 [0.1193] & 0.951 [0.1272] \\
10000 & CC & PDR--CV2 & 0.944 [0.1154] & 0.942 [0.1093] & 0.950 [0.1051] & 0.947 [0.1028] & 0.948 [0.1022] & 0.949 [0.1028] & 0.948 [0.1050] & 0.949 [0.1093] & 0.950 [0.1153] \\
10000 & CC & ProxLL--US & 0.944 [0.1818] & 0.946 [0.1664] & 0.950 [0.1551] & 0.951 [0.1494] & 0.951 [0.1476] & 0.952 [0.1493] & 0.951 [0.1552] & 0.952 [0.1662] & 0.955 [0.1817] \\
10000 & MC & PDR--PI1 & 0.955 [0.3418] & 0.952 [0.3015] & 0.947 [0.2714] & 0.949 [0.2556] & 0.949 [0.2517] & 0.946 [0.2559] & 0.950 [0.2716] & 0.949 [0.3015] & 0.953 [0.3420] \\
10000 & MC & PDR--PI2 & 0.956 [0.4185] & 0.952 [0.3688] & 0.949 [0.3315] & 0.949 [0.3123] & 0.948 [0.3072] & 0.949 [0.3126] & 0.952 [0.3318] & 0.954 [0.3687] & 0.953 [0.4186] \\
10000 & MC & PDR--CV1 & 0.959 [0.3135] & 0.954 [0.2767] & 0.946 [0.2493] & 0.945 [0.2349] & 0.947 [0.2312] & 0.950 [0.2351] & 0.953 [0.2494] & 0.947 [0.2767] & 0.951 [0.3135] \\
10000 & MC & PDR--CV2 & 0.961 [0.2645] & 0.955 [0.2341] & 0.948 [0.2114] & 0.942 [0.1995] & 0.944 [0.1964] & 0.948 [0.1996] & 0.949 [0.2116] & 0.950 [0.2341] & 0.951 [0.2645] \\
10000 & MC & ProxLL--US & 0.956 [0.4570] & 0.953 [0.4020] & 0.954 [0.3613] & 0.950 [0.3398] & 0.953 [0.3347] & 0.954 [0.3405] & 0.953 [0.3614] & 0.956 [0.4021] & 0.953 [0.4568] \\
10000 & CM & PDR--PI1 & 0.949 [0.1447] & 0.942 [0.1345] & 0.949 [0.1270] & 0.946 [0.1229] & 0.944 [0.1214] & 0.951 [0.1219] & 0.948 [0.1248] & 0.948 [0.1307] & 0.952 [0.1389] \\
10000 & CM & PDR--PI2 & 0.950 [0.1533] & 0.945 [0.1419] & 0.951 [0.1335] & 0.948 [0.1289] & 0.948 [0.1273] & 0.955 [0.1278] & 0.953 [0.1311] & 0.947 [0.1376] & 0.954 [0.1468] \\
10000 & CM & PDR--CV1 & 0.949 [0.1263] & 0.942 [0.1188] & 0.951 [0.1132] & 0.949 [0.1102] & 0.949 [0.1092] & 0.952 [0.1095] & 0.950 [0.1117] & 0.950 [0.1160] & 0.952 [0.1221] \\
10000 & CM & PDR--CV2 & 0.943 [0.1146] & 0.940 [0.1089] & 0.949 [0.1047] & 0.947 [0.1024] & 0.947 [0.1017] & 0.948 [0.1020] & 0.950 [0.1036] & 0.951 [0.1069] & 0.952 [0.1115] \\
10000 & CM & ProxLL--US & 0.947 [0.1816] & 0.944 [0.1666] & 0.951 [0.1554] & 0.951 [0.1493] & 0.951 [0.1469] & 0.952 [0.1476] & 0.952 [0.1520] & 0.951 [0.1607] & 0.954 [0.1729] \\
10000 & MM & PDR--PI1 & 0.054 [0.3180] & 0.133 [0.2857] & 0.451 [0.2608] & 0.874 [0.2468] & 0.918 [0.2420] & 0.575 [0.2435] & 0.143 [0.2531] & 0.034 [0.2724] & 0.014 [0.2988] \\
10000 & MM & PDR--PI2 & 0.143 [0.3881] & 0.294 [0.3484] & 0.614 [0.3177] & 0.904 [0.3005] & 0.935 [0.2945] & 0.705 [0.2964] & 0.296 [0.3081] & 0.086 [0.3319] & 0.029 [0.3644] \\
10000 & MM & PDR--CV1 & 0.026 [0.2909] & 0.090 [0.2615] & 0.392 [0.2389] & 0.863 [0.2261] & 0.914 [0.2217] & 0.529 [0.2230] & 0.095 [0.2318] & 0.015 [0.2493] & 0.004 [0.2732] \\
10000 & MM & PDR--CV2 & 0.010 [0.2456] & 0.036 [0.2213] & 0.250 [0.2026] & 0.827 [0.1919] & 0.897 [0.1883] & 0.389 [0.1894] & 0.040 [0.1966] & 0.006 [0.2111] & 0.002 [0.2309] \\
10000 & MM & ProxLL--US & 0.201 [0.4242] & 0.351 [0.3804] & 0.655 [0.3466] & 0.913 [0.3276] & 0.939 [0.3213] & 0.725 [0.3232] & 0.346 [0.3363] & 0.132 [0.3623] & 0.067 [0.3984] \\


==> tables/simulation/cv-edge-rows.tex <==
% Sources: frozen CV diagnostics in configuration 4e7d28a1 and ProxLQ-CV1 diagnostics in configuration 0bebf0fb.
% Schema: estimand & selector & max lower-bound hit rate & max upper-bound hit rate & max boundary hit rate & max terminal-decreasing rate & max selected-invalid fraction & min selected neighbors & min selected pivot ratio & max mean density-floor fraction \\
% Scope: extrema over n in {2500,5000,7500,10000} and scenarios CC, CM, MC, and MM; 5000 replications per cell.
% Rounding: rates through selected-invalid fraction use four decimals; pivot ratios and density-floor fractions use six decimals.
% -- denotes a diagnostic that is not defined for the dose-response selector.
Dose response & PDR--CV1 & 0.0000 & 0.7556 & 0.7556 & 0.8246 & 0.0000 & -- & -- & 0.000000 \\
Dose response & PDR--CV2 & 0.0004 & 0.7056 & 0.7058 & 0.8002 & 0.0000 & -- & -- & 0.000000 \\
Dose response & ProxLL--CV1 & 0.0030 & 0.4028 & 0.4048 & 0.4988 & 0.0000 & -- & -- & 0.000000 \\
Derivative & PDR--CV1 & 0.2418 & 0.0254 & 0.2524 & 0.5460 & 0.0000 & 89 & 0.006115 & 0.000460 \\
Derivative & PDR--CV2 & 0.2300 & 0.0136 & 0.2372 & 0.5294 & 0.0000 & 138 & 0.005721 & 0.000460 \\
Derivative & ProxLQ--CV1 & 0.2602 & 0.0186 & 0.2684 & 0.5170 & 0.0000 & 90 & 0.028262 & 0.000460 \\
\bottomrule


==> tables/simulation/parametric-null-power.tex <==
\begin{landscape}
\begingroup
\color{OliveGreen}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{.96}
\begin{longtable}{lr*{7}{r}}
\caption{\color{OliveGreen}Mean fixed-departure rejection probability by canonical method and sample size. Entries are unweighted means over the three nulls and CC, CM, and MC. Values are not adjusted for empirical size.}
\label{tab:sim-parametric-null-power} \\
\toprule
Method & $n$ & $.004$ & $.008$ & $.012$ & $.016$ & $.024$ & $.040$ & $.080$ \\
\midrule
\endfirsthead
\caption[]{\color{OliveGreen}Mean fixed-departure rejection probability by canonical method and sample size. (continued).} \\
\toprule
Method & $n$ & $.004$ & $.008$ & $.012$ & $.016$ & $.024$ & $.040$ & $.080$ \\
\midrule
\endhead
\midrule \multicolumn{9}{r}{Continued on next page} \\
\endfoot
\bottomrule
\endlastfoot
PDR--PI1 & $2{,}500$ & .061 & .077 & .116 & .177 & .400 & .884 & 1.000 \\
PDR--PI1 & $5{,}000$ & .064 & .099 & .185 & .346 & .726 & .992 & 1.000 \\
PDR--PI1 & $7{,}500$ & .062 & .110 & .267 & .536 & .891 & .999 & 1.000 \\
PDR--PI1 & $10{,}000$ & .083 & .164 & .370 & .661 & .956 & 1.000 & 1.000 \\
PDR--PI2 & $2{,}500$ & .055 & .068 & .095 & .138 & .314 & .812 & 1.000 \\
PDR--PI2 & $5{,}000$ & .064 & .086 & .140 & .254 & .597 & .977 & 1.000 \\
PDR--PI2 & $7{,}500$ & .054 & .088 & .197 & .407 & .820 & .999 & 1.000 \\
PDR--PI2 & $10{,}000$ & .076 & .137 & .294 & .540 & .911 & 1.000 & 1.000 \\
PDR--CV1 & $2{,}500$ & .062 & .084 & .130 & .203 & .463 & .921 & 1.000 \\
PDR--CV1 & $5{,}000$ & .063 & .107 & .214 & .391 & .793 & .996 & 1.000 \\
PDR--CV1 & $7{,}500$ & .062 & .129 & .317 & .595 & .926 & 1.000 & 1.000 \\
PDR--CV1 & $10{,}000$ & .086 & .181 & .420 & .720 & .972 & 1.000 & 1.000 \\
PDR--CV2 & $2{,}500$ & .066 & .097 & .164 & .273 & .593 & .956 & 1.000 \\
PDR--CV2 & $5{,}000$ & .074 & .136 & .282 & .505 & .872 & 1.000 & 1.000 \\
PDR--CV2 & $7{,}500$ & .072 & .175 & .419 & .699 & .961 & 1.000 & 1.000 \\
PDR--CV2 & $10{,}000$ & .096 & .227 & .532 & .822 & .986 & 1.000 & 1.000 \\
ProxLL--raw & $2{,}500$ & .063 & .107 & .197 & .333 & .691 & .978 & 1.000 \\
ProxLL--raw & $5{,}000$ & .078 & .159 & .353 & .609 & .925 & .999 & 1.000 \\
ProxLL--raw & $7{,}500$ & .077 & .219 & .527 & .785 & .980 & 1.000 & 1.000 \\
ProxLL--raw & $10{,}000$ & .106 & .292 & .652 & .889 & .995 & 1.000 & 1.000 \\
ProxLL--US & $2{,}500$ & .054 & .067 & .091 & .141 & .307 & .789 & .999 \\
ProxLL--US & $5{,}000$ & .060 & .081 & .136 & .251 & .587 & .966 & 1.000 \\
ProxLL--US & $7{,}500$ & .051 & .086 & .182 & .373 & .791 & .997 & 1.000 \\
ProxLL--US & $10{,}000$ & .069 & .127 & .269 & .517 & .896 & .999 & 1.000 \\
\end{longtable}
\endgroup
\end{landscape}
\clearpage

\begin{landscape}
\begingroup
\color{OliveGreen}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{.82}
\begin{longtable}{lll*{7}{r}}
\caption{\color{OliveGreen}Mean fixed-departure rejection probability by null, scenario, and sample size. Entries are unweighted means over the six canonical methods. Values are not adjusted for empirical size.}
\label{tab:sim-parametric-null-power-scenario} \\
\toprule
Scenario & Null & $n$ & $.004$ & $.008$ & $.012$ & $.016$ & $.024$ & $.040$ & $.080$ \\
\midrule
\endfirsthead
\caption[]{\color{OliveGreen}Mean fixed-departure rejection probability by null, scenario, and sample size. (continued).} \\
\toprule
Scenario & Null & $n$ & $.004$ & $.008$ & $.012$ & $.016$ & $.024$ & $.040$ & $.080$ \\
\midrule
\endhead
\midrule \multicolumn{10}{r}{Continued on next page} \\
\endfoot
\bottomrule
\endlastfoot
CC & constant & $2{,}500$ & .056 & .084 & .145 & .242 & .548 & .966 & 1.000 \\
CC & constant & $5{,}000$ & .073 & .128 & .257 & .468 & .849 & .999 & 1.000 \\
CC & constant & $7{,}500$ & .065 & .146 & .377 & .670 & .971 & 1.000 & 1.000 \\
CC & constant & $10{,}000$ & .087 & .206 & .485 & .790 & .994 & 1.000 & 1.000 \\
CC & linear & $2{,}500$ & .056 & .086 & .145 & .244 & .551 & .966 & 1.000 \\
CC & linear & $5{,}000$ & .072 & .125 & .259 & .476 & .856 & .999 & 1.000 \\
CC & linear & $7{,}500$ & .064 & .153 & .385 & .678 & .970 & 1.000 & 1.000 \\
CC & linear & $10{,}000$ & .087 & .215 & .504 & .798 & .993 & 1.000 & 1.000 \\
CC & quadratic & $2{,}500$ & .060 & .088 & .139 & .224 & .500 & .944 & 1.000 \\
CC & quadratic & $5{,}000$ & .070 & .119 & .235 & .426 & .821 & .999 & 1.000 \\
CC & quadratic & $7{,}500$ & .067 & .146 & .349 & .628 & .956 & 1.000 & 1.000 \\
CC & quadratic & $10{,}000$ & .087 & .197 & .463 & .757 & .987 & 1.000 & 1.000 \\
CM & constant & $2{,}500$ & .060 & .087 & .153 & .257 & .574 & .974 & 1.000 \\
CM & constant & $5{,}000$ & .072 & .129 & .267 & .488 & .865 & 1.000 & 1.000 \\
CM & constant & $7{,}500$ & .068 & .161 & .390 & .693 & .976 & 1.000 & 1.000 \\
CM & constant & $10{,}000$ & .088 & .215 & .506 & .810 & .994 & 1.000 & 1.000 \\
CM & linear & $2{,}500$ & .056 & .088 & .154 & .263 & .575 & .975 & 1.000 \\
CM & linear & $5{,}000$ & .070 & .130 & .276 & .495 & .870 & 1.000 & 1.000 \\
CM & linear & $7{,}500$ & .066 & .163 & .408 & .710 & .975 & 1.000 & 1.000 \\
CM & linear & $10{,}000$ & .092 & .221 & .522 & .820 & .995 & 1.000 & 1.000 \\
CM & quadratic & $2{,}500$ & .063 & .088 & .146 & .233 & .519 & .955 & 1.000 \\
CM & quadratic & $5{,}000$ & .068 & .121 & .243 & .452 & .833 & .999 & 1.000 \\
CM & quadratic & $7{,}500$ & .068 & .152 & .363 & .647 & .962 & 1.000 & 1.000 \\
CM & quadratic & $10{,}000$ & .087 & .211 & .482 & .775 & .991 & 1.000 & 1.000 \\
MC & constant & $2{,}500$ & .069 & .083 & .113 & .158 & .307 & .763 & 1.000 \\
MC & constant & $5{,}000$ & .060 & .089 & .149 & .255 & .571 & .971 & 1.000 \\
MC & constant & $7{,}500$ & .059 & .102 & .201 & .367 & .759 & .999 & 1.000 \\
MC & constant & $10{,}000$ & .087 & .146 & .289 & .502 & .885 & 1.000 & 1.000 \\
MC & linear & $2{,}500$ & .064 & .078 & .104 & .145 & .296 & .747 & 1.000 \\
MC & linear & $5{,}000$ & .059 & .082 & .141 & .245 & .563 & .970 & 1.000 \\
MC & linear & $7{,}500$ & .056 & .096 & .201 & .360 & .757 & .998 & 1.000 \\
MC & linear & $10{,}000$ & .081 & .144 & .288 & .498 & .879 & .999 & 1.000 \\
MC & quadratic & $2{,}500$ & .057 & .068 & .090 & .131 & .282 & .721 & .999 \\
MC & quadratic & $5{,}000$ & .059 & .079 & .136 & .227 & .522 & .957 & 1.000 \\
MC & quadratic & $7{,}500$ & .053 & .090 & .189 & .339 & .727 & .996 & 1.000 \\
MC & quadratic & $10{,}000$ & .077 & .137 & .267 & .474 & .856 & .999 & 1.000 \\
\end{longtable}
\endgroup
\end{landscape}
\clearpage


==> tables/simulation/pointwise-grid-rows.tex <==
% n & scenario & PDR-PI1 & PDR-PI2 & PDR-CV1 & PDR-CV2 & ProxLL-US; coverage [mean width]
2500 & CC & 0.9481 [0.241] & 0.9508 [0.252] & 0.9494 [0.218] & 0.9478 [0.204] & 0.9511 [0.276] \\
2500 & CM & 0.9477 [0.239] & 0.9507 [0.248] & 0.9495 [0.216] & 0.9476 [0.202] & 0.9506 [0.273] \\
2500 & MC & 0.9479 [0.501] & 0.9495 [0.601] & 0.9477 [0.462] & 0.9463 [0.394] & 0.9507 [0.622] \\
5000 & CC & 0.9513 [0.176] & 0.9528 [0.185] & 0.9518 [0.158] & 0.9519 [0.147] & 0.9525 [0.209] \\
5000 & CM & 0.9508 [0.174] & 0.9526 [0.183] & 0.9514 [0.157] & 0.9516 [0.146] & 0.9526 [0.206] \\
5000 & MC & 0.9491 [0.373] & 0.9503 [0.454] & 0.9489 [0.344] & 0.9497 [0.293] & 0.9522 [0.481] \\
7500 & CC & 0.9472 [0.147] & 0.9489 [0.155] & 0.9474 [0.132] & 0.9463 [0.122] & 0.9502 [0.178] \\
7500 & CM & 0.9467 [0.146] & 0.9488 [0.153] & 0.9472 [0.130] & 0.9459 [0.121] & 0.9502 [0.176] \\
7500 & MC & 0.9490 [0.316] & 0.9507 [0.385] & 0.9494 [0.291] & 0.9500 [0.247] & 0.9523 [0.415] \\
10000 & CC & 0.9478 [0.129] & 0.9500 [0.137] & 0.9483 [0.115] & 0.9474 [0.106] & 0.9511 [0.159] \\
10000 & CM & 0.9474 [0.128] & 0.9497 [0.135] & 0.9485 [0.114] & 0.9476 [0.105] & 0.9511 [0.157] \\
10000 & MC & 0.9499 [0.281] & 0.9513 [0.343] & 0.9502 [0.258] & 0.9491 [0.219] & 0.9530 [0.374] \\
\bottomrule

